Fault Localization via Fine-tuning Large Language Models with Mutation Generated Stack Traces

Abrupt and unexpected terminations of software are termed as software crashes. They can be challenging to analyze. Finding the root cause requires extensive manual effort and expertise to connect information sources like stack traces, source code, and logs. Typical approaches to fault localization require either test failures or source code. Crashes occurring in production environments, such as that of SAP HANA, provide solely crash logs and stack traces. We present a novel approach to localize faults based only on the stack trace information and no additional runtime information, by fine-tuning large language models (LLMs). We address complex cases where the root cause of a crash differs from the technical cause, and is not located in the innermost frame of the stack trace. As the number of historic crashes is insufficient to fine-tune LLMs, we augment our dataset by leveraging code mutators to inject synthetic crashes into the code base. By fine-tuning on 64,369 crashes resulting from 4.1 million mutations of the HANA code base, we can correctly predict the root cause location of a crash with an accuracy of 66.9\% while baselines only achieve 12.6% and 10.6%. We substantiate the generalizability of our approach by evaluating on two additional open-source databases, SQLite and DuckDB, achieving accuracies of 63% and 74%, respectively. Across all our experiments, fine-tuning consistently outperformed prompting non-finetuned LLMs for localizing faults in our datasets.

==> evaluation.tex <==
\section{Evaluation}


==> introduction_2.tex <==
\subsection{New introduction}
 


The authors note that such bug reports containing stack traces or logs are more likely to be resolved earlier as per studies in  -- cite the papers from Thesis

As a initial step to triage a bug, an automatic FL located to assess the stack traces located in the bug report may reduce the time required to solve the bug??


When debugging
user-reported bugs, logs (i.e., either log snippets, stack traces, or both) are
usually the only source of information that is available to developers


Developers need to manually analyze the logs to diagnose the problem. Hence, if the attached logs are unclear or insufficient, debugging can become even more time consuming and challenging.




CAN YOU CITE A PHD THESIS 




PREPROCESSING:



DATA: 





==> metrics.tex <==
%\begin{itemize}
    %\item ROUGE: Recall-Oriented Understudy for Gisting Evaluation is referred to as ROUGE. It includes measures to compare the quality of a prediction to the expected outcome. 
    %\item Perplexity: Its is the average of the log likelihood for the sequence of the tokens for a given model. It is a statistical measure of how well the model is capable of predicting a sequence of tokens. Lower the perplexity better the model at predicting the sequence.
    %\item BLEU score: Is a precision based score and measures how similar the generated text is to a reference.It is a weighted average to combine the precision scores for various n-gram sizes by taking their geometric mean. Longer n-grams are typically given more weight because they capture more significant phrases.
    %It  To get the overall quality of the prediction, the scores are then averaged across the entire corpus. 
    %\item Accuracy@K: For a given failure, we predict multiple fault locations, and if one of the strings from K predictions matches the ground truth exactly, we consider that prediction to be accurate. For the evaluation, we average performance across the dataset.
%\end{itemize}


% This doesn't deserve its own separate file anymore :D


We present an average accuracy for both the baseline and the finetuned LLM across all mutation and crash types within our dataset.
Additionally, we calculate averages for precision, recall, and F1-Score to measure the model's overall performance.


\textit{Accuracy}: We consider a target accurately predicted when the predicted tokens excluding the end-of-generation token, $A$, perfectly match the target tokens, $B$ as shown in \Cref{eq: Match} and calculate accuracy over the dataset .
as shown in \Cref{eq: Accuracy}.\\
$A$ is a concatenation of a sequence of predicted tokens excluding the end-of-generation token and $B$ is the target function name.
\[A = \bigcup_{a \in A', a \neq X} a\] where $A'$ = \((a_1, \ldots, a_m, \textsc{'<|endoftext|>'})\), $X=\textsc{'<|endoftext|>'}$


\begin{equation}
\text{Match}(A, B) =
\begin{cases} 
1 & \text{if } A = B \\
0 & \text{otherwise}
\end{cases}
\label{eq: Match}
\end{equation}


\begin{equation}
\text{Accuracy} = \frac{1}{N} \sum_{i=1}^{N} \text{Match}(A_i, B_i)
\label{eq: Accuracy}
\end{equation}
where $N$ is the total number of predictions and ($A_i$, $B_i$) are (predicted, actual) of the $i^{th}$ prediction.\\

%\ncj{Address MM comments here!}
 %Moritz: I don't understand the defintion of TP and FP.
 % I woud also introduce A and B as tuples with N entries A = (a1, ...ai, a_n{pred_count})  and B = (b1, ..., bi, ..b_{n}).
 % So the prediction and the group truth can have and usually have a different amount of tokens N_{pred_count} != N_{gt}. 
 % First case N_{pred_count} < N_{gt}: The ground truth B has more tokens than the predicted tokens A. Hence, you get 100% if you just predict a subset, as you only iterating over the number of predicted tokens.
 % Second cae N_{pred_count} > N_{gt}: So are all Macthes ignored if the current index "i" is larger than N_{gt}?
 % Moreover, TP() is a fucntion that takes c as an input? What about A and B. I did not understand what is the difference of c to A and B. If c is a class, is it a predicted class or the ground truth class?
 % If c is a class, how c_i then defined? The A, B matching makes sense to me, but you lost me on this additional c part. I think it should be introduced and explained, what the difference to A and B.

 $True\ Positive$ (TP) represents predictions  where samples from class $B$ are correctly classified. $False\ Positive$ (FP)  represents predictions where samples from other classes are incorrectly attributed to class $B$. $False\ Negative$ (FN)  represents  predictions where samples from class $B$  are incorrectly attributed to other classes.\\
 
% \begin{equation}
% \text{TP}(B) = \sum_{i=1}^{N} \left\{
% \begin{array}{ll}
% 1 & \text{if } A_i = B \text{ and Match}(A_i, B_i) = 1 \\
% 0 & \text{otherwise}
% \end{array}
% \right.
% \label{eq: TP}
% \end{equation}


% \begin{equation}
% \text{FP}(B) = \sum_{i=1}^{N} \left\{
% \begin{array}{ll}
% 1 & \text{if } A_i = B \text{ and Match}(A_i, B_i) = 0 \\
% 0 & \text{otherwise}
% \end{array}
% \right.
% \label{eq: FP}
% \end{equation}

% \begin{equation}
% \text{FN}(B) = \sum_{i=1}^{N} \left\{
% \begin{array}{ll}
% 1 & \text{if } A_i \neq B \text{ and Match}(A_i, B_i) = 0 \\
% 0 & \text{otherwise}
% \end{array}
% \right.
% \label{eq: FN}
% \end{equation}







 % MOritz: Thumb rule. Avoid past tense. -->: It meassures the prediction precision/accuracy of class c .
\textit{Precision}: The ratio of true positive predictions to the total positive predictions generated by the model for a given class. % A measure of how many of the predictions made by a model for a class are actually correct.
  \begin{equation}
\text{Precision}(B) = \frac{\text{TP}(B)}{\text{TP}(B) + \text{FP}(B)}
\label{eq: Precision}
\end{equation}

% \begin{equation}
% \text{Precision(c)} = \frac{1}{N_c} \sum_{i=1}^{N_c} \text{Match}(A_i, B_i)
% \end{equation}
% where $N_c = True\ positive + False\ positive$ for class $c$. \\ 
% Moritz: I think you can also just mention the definition of Recall and Precision, as it is much harder to describe it by words.
\textit{Recall}:  The ratio of true positive predictions to the total number of actual positive instances of a given class in the dataset. % A measure of how many of the total number of instances of a given class in the dataset were correctly identified by the model.


\begin{equation}
\text{Recall}(B) = \frac{\text{TP}(B)}{\text{TP}(B) + \text{FN}(B)}
\label{eq: Recall}
\end{equation}

\textit{F1-Score}: Is the harmonic mean of precision and recall is calculated using the following formula:
\begin{equation}
\text{F1-Score}(B) = \frac{2 \cdot \text{Precision}(B) \cdot \text{Recall}(B)}{\text{Precision}(B) + \text{Recall}(B)}
\label{eq: F1Measure}
\end{equation}


 The average of F1-scores across all classes offers a comprehensive evaluation of the model's performance.

% \begin{equation}
% \text{Recall} = \frac{\text{True Positives}}{\text{True Positives} + \text{False Negatives}}
% \end{equation}

% should we connect why we choose these 3?
% While accuracy provides an overview of the model's performance, precision and recall can present a granular overview of performance for a given class and play a particularly important role in imbalanced datasets. 

